Uncovering Adversarial Risks of Test-Time Adaptation

Recently, test-time adaptation (TTA) has been proposed as a promising solution for addressing distribution shifts. It allows a base model to adapt to an unforeseen distribution during inference by leveraging the information from the batch of (unlabeled) test data. However, we uncover a novel security vulnerability of TTA based on the insight that predictions on benign samples can be impacted by malicious samples in the same batch. To exploit this vulnerability, we propose Distribution Invading Attack (DIA), which injects a small fraction of malicious data into the test batch. DIA causes models using TTA to misclassify benign and unperturbed test data, providing an entirely new capability for adversaries that is infeasible in canonical machine learning pipelines. Through comprehensive evaluations, we demonstrate the high effectiveness of our attack on multiple benchmarks across six TTA methods. In response, we investigate two countermeasures to robustify the existing insecure TTA implementations, following the principle of "security by design". Together, we hope our findings can make the community aware of the utility-security tradeoffs in deploying TTA and provide valuable insights for developing robust TTA approaches.

==> Table/all_corr_fig.tex <==

% \begin{table}[H]
% \centering
% \refstepcounter{table}
% \resizebox{0.8\columnwidth}{!}{%
% \begin{tabular}{cc|cc} 
% \toprule 
%  \makecell{ \textbf{(a) Snow Corruption} } &
%  \makecell{ \textbf{(b) Snow Attack} }  & 
%  \makecell{ \textbf{(c) Fog Corruption} } & 
%  \makecell{ \textbf{(d) Fog Attack} }\\
%  \midrule
%  \includegraphics[width=0.19\textwidth]
%  {Figures/common_corr/ILSVRC2012_val_00000003.png}  & 
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/snowsnow6180.png}  &
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/ILSVRC2012_val_000000032.png}  & 
%  \includegraphics[width=0.19\textwidth]
%  {Figures/common_corr/fogfog180.png} \\
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/ILSVRC2012_val_000002932.png}  & 
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/snowsnow6181.png}  &
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/ILSVRC2012_val_00000293.png}  & 
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/fogfog181.png}  \\
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/ILSVRC2012_val_000004142.png} & 
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/snowsnow6182.png} &
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/ILSVRC2012_val_00000414.png}& 
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/fogfog182.png}\\
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/ILSVRC2012_val_000006512.png}& 
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/snowsnow6183.png} &
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/ILSVRC2012_val_00000651.png} & 
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/fogfog183.png} \\ 
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/ILSVRC2012_val_000009212.png}& 
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/snowsnow6184.png} &
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/ILSVRC2012_val_00000921.png} & 
%  \includegraphics[width=0.19\textwidth]{Figures/common_corr/fogfog184.png} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Demonstrations of the corrupted fog and snow dataset from ImageNet-C and adversarially corrupted images (malicious DIA). We observe that manually distinguishing malicious and benign samples is hard. }
% \label{Tab:IN_CORR}
% \end{table}



\begin{figure}[H]
\centering
\includegraphics{Figures/common_corr/imagecorr.png}
\caption{Demonstrations of the corrupted fog and snow dataset from ImageNet-C and adversarially corrupted images (malicious DIA). We observe that manually distinguishing malicious and benign samples is hard. }
\label{Tab:IN_CORR}
\end{figure}



==> Table/arch_table_full.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[H]
\centering
\caption{ Effectiveness of distribution invading attack across various model architectures and data augmentations. (CIAFR-C: $N_m$=40; ImageNet-C: $N_m$=10)}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Architectures} & \textbf{TeBN} & \textbf{TENT} & \textbf{Hard PL} & \textbf{Soft PL} & \textbf{Robust PL} & \textbf{Conjugate PL} \\ \midrule
\multirow{3}{*}{\textbf{CIFAR-10-C}}  & ResNet26 \cite{He2016DeepRL}      & 92.80 & 83.87 &   84.27 &   82.93 & 86.93 &      85.47 \\
                                      & VGG \cite{Simonyan2015VeryDC}     & 79.07 & 65.33 &   67.47 &   64.13 & 67.47 &      64.13 \\
                                      & WRN28  \cite{Zagoruyko2016WideRN} & 93.73 & 89.60 &   90.80 &   90.13 & 91.20 &      89.33 \\ \midrule
\multirow{3}{*}{\textbf{CIFAR-100-C}}  & ResNet26 \cite{He2016DeepRL}       & 100.00 & 100.00 &   99.87 &  100.00 & 99.87 &     100.00 \\
                                      & VGG    \cite{Simonyan2015VeryDC}    &  88.00 &  82.93 &   86.53 &   85.73 & 87.33 &      85.47 \\
                                      & WRN28  \cite{Zagoruyko2016WideRN}   &  97.47 &  83.60 &   87.07 &   86.67 & 90.13 &      79.73 \\
                                      \toprule
\textbf{Dataset} & \textbf{Augmentations} & \textbf{TeBN} & \textbf{TENT} & \textbf{Hard PL} & \textbf{Soft PL} & \textbf{Robust PL} & \textbf{Conjugate PL} \\ \midrule
\multirow{3}{*}{\textbf{ImageNet-C}}  &  Standard \cite{He2016DeepRL}          & 99.47 & 97.07 &   96.53 &   94.13 & 96.00 &      92.80 \\
                                      & AugMix  \cite{Hendrycks2020AugMixAS}   & 98.40 & 94.13 &   93.60 &   88.27 & 92.00 &      87.20 \\
                                      & DeepAugment \cite{Hendrycks2021TheMF}  & 96.00 & 92.00 &   91.20 &   87.47 & 89.60 &      86.67 \\                                  
\bottomrule
\end{tabular}%
}
\label{tab:arch_full}
\end{table}

==> Table/backup.tex <==
\begin{figure}[H]
\begin{center}
\begin{tabular}{cc}
\subfigure{
\label{Tab:IN_Constrained.sub.f1}
\includegraphics[width=0.13\textwidth]{Figures/epsilon/image16/testori_eps0.0627451000.png}}
\subfigure{
\label{Tab:IN_Constrained.sub.f2}
\includegraphics[width=0.13\textwidth]{Figures/constrained_figs/testeps199.png}}
\subfigure{
\label{Tab:IN_Constrained.sub.f3}
\includegraphics[width=0.13\textwidth]{Figures/epsilon/image16/testadv_eps0.0627451000.png}}
&
\subfigure{
\label{Tab:IN_Constrained.sub.1}
\includegraphics[width=0.13\textwidth]{Figures/constrained_figs/adv1.png}}
\subfigure{
\label{Tab:IN_Constrained.sub.2}
\includegraphics[width=0.13\textwidth]{Figures/constrained_figs/snowsnow6180.png}}
\subfigure{
\label{Tab:IN_Constrained.sub.3}
\includegraphics[width=0.13\textwidth]{Figures/constrained_figs/fogfog180.png}}
\\
(a) & (b)
\end{tabular}
\caption{(a) An example of the eyeglass frame attack.  Left: original face input image.  Middle: modified input image (adversarial eyeglasses superimposed on the face).  Right: an image of the predicted individual with the adversarial input in the middle image. 
(b) An example of the stop sign attack.  Left: original stop sign input image.  Middle: adversarial mask.  Right: stop sign image with adversarial stickers, classified as a speed limit sign.}
\label{Tab:IN_Constrained}
\end{center}
\end{figure}

==> Table/robust_corr.tex <==
\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
\textbf{Dataset} & \textbf{ Models}  & \textbf{Source} & \textbf{TeBN} & \textbf{TENT} & \textbf{Hard PL} & \textbf{Soft PL} & \textbf{Robust PL} & \textbf{Conjugate PL} \\ \midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}CIFAR-10-C\\ (ResNet26)\end{tabular}}}  
& Standard &  74.92 & 86.50 & 87.59 &   87.23 &   87.44 & 86.89 &      88.00 \\
& \cite{Gowal2021ImprovingRU}   & 79.10 & 83.22 & 90.78 &   88.84 &   91.07 & 91.15 &      89.65 \\
& \cite{Wu2020AdversarialWP}   &   79.55 & 84.86 & 86.03 &   85.86 &   86.02 & 85.88 &      86.08 \\
 \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}CIFAR-100-C\\ (ResNet26)\end{tabular}}} 
& 0   &    65.94 & 67.12 &   65.75 &   66.75 & 65.20 &      68.17\\
& 10  &    56.16 & 57.10 &   55.35 &   56.55 & 54.66 &      57.99 \\
& 20  &    48.01 & 49.67 &   48.00 &   49.20 & 47.48 &      50.61 \\
\hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}ImageNet-C\\ (ResNet50)\end{tabular}}}  
& 0 &   52.18 & 55.99 &   56.51 &   58.12 & 57.05 &      58.48  \\ 
& 5 &  41.53 & 45.82 &   46.59 &   48.71 & 47.55 &      49.05 \\
& 10 &  31.61 & 37.89 &   39.27 &   42.31 & 40.88 &      42.97 \\
                                                                                           \bottomrule
\end{tabular}%
}
\caption{Average corruption accuracy of multiple corruption types when deploying distribution invading attack on overall performance. As a reference, 10 malicious data represent 5\% of input. tw{Experiments running ...}}
\label{tab:robust_corr}
\end{table}

==> Table/unknown_para.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table}[t]
% \centering
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{@{}ccccccccc@{}}
% \toprule
% \textbf{Dataset} & \textbf{Architectures }& \textbf{Known} & \textbf{TeBN(\%)} & \textbf{TENT(\%)} & \textbf{Hard PL(\%)} & \textbf{Soft PL(\%)} & \textbf{Robust PL(\%)} & \textbf{Conjugate PL(\%)}  \\ \midrule
% \multirow{2}{*}{\textbf{CIFAR-10-C}}  
% & \multirow{2}{*}{ ResNet26   } 
% & All   & 92.80 & 83.87 &   84.27 &   82.93 & 86.93 &      85.47 \\
% & & Initial    & 92.80 & 64.27 &   68.67 &   65.73 & 72.80 &      62.40 \\
%                                        \midrule
% \multirow{2}{*}{\textbf{CIFAR-100-C}}  
% & \multirow{2}{*}{ ResNet26   } 
% &  All & 100.00 & 100.00 &   99.87 &  100.00 & 99.87 &     100.00 \\
% & &  Initial  & 100.00 & 34.53 &   42.53 &   37.60 & 44.67 &      31.73\\
%  \midrule
% \multirow{2}{*}{\textbf{ImageNet-C}}  
% & \multirow{2}{*}{ ResNet50    } 
% &  All  & 99.47 & 97.07 &   96.53 &   94.13 & 96.00 &      92.80 \\       
% & &  Initial   &  99.47 & 79.20 &   68.27 &   53.07 & 62.13 &      48.53
%  \\                             
% \bottomrule
% \end{tabular}%
% }
% \caption{ Effectiveness of distribution invading attack with the knowledge of Initial model parameters only. [CIAFR-C: $N_m$=40 ; ImageNet-C: $N_m$=10]}
% \label{tab:unknown_para}
% \end{table}




\begin{table}[t]
\centering
  \vspace{-5mm}
\caption{ Effectiveness of Distribution Invading Attack with the knowledge of Initial model parameters only. Table \ref{tab:unknown_para_all} presents full results. [CIAFR-C: $N_m$=40 ; ImageNet-C: $N_m$=10]}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Dataset/Model}& \textbf{Knowledge} & \textbf{TeBN(\%)} & \textbf{TENT(\%)} & \textbf{Hard PL(\%)}  \\ \midrule
CIFAR-10-C/ & $\preparam$   & 92.80 & 83.87 &   84.27 \\
ResNet-26   & $\srcparam$    & 92.80 & 64.27 &   68.67 \\
                                       \midrule

CIFAR-100-C/ &  $\preparam$  & 100.00 & 100.00 &   99.87  \\
ResNet-26    &  $\srcparam$  & 100.00 & 34.53 &   42.53 \\
 \midrule

ImageNet-C/  & $\preparam$   &  99.47 & 98.67 &   96.53 \\       
ResNet-50    & $\srcparam$   &  99.47 & 79.20 &   68.27 \\                       
\bottomrule
\vspace{-5mm}
\end{tabular}%
}
\label{tab:unknown_para}
\end{table}
    
    
    

==> robustBN.tex <==

% \smallskip \noindent \textbf{Leveraging Median  Batch Norm Statistics.} \smallskip \noindent Use $1-\alpha$ source BN statistics + $\alpha$ test BN statistics(median, mad)


\subsubsection{Does Robust Statistics help for better BN Estimation?}


In this subsection, we seek to alleviate all vulnerable information derived from test-time BN completely. 
Therefore, we consider replacing mean and standard deviation with the median $M_t$ and median absolute deviation (MAD) \cite{Leys2013DetectingOD}. 
However, one concern of adopting median and MAD is that inconsistent estimation of BN between the training and test stages might result in large performance degradation. 
Therefore, we consider combining it with training-time BN and layer-wise BN, which can be formulated as: 

\begin{equation}
    \bar{\mu}= \tau \mu_s+ (1-\tau) M_t, \quad \bar{\sigma}^2=\tau \sigma_s^2+(1-\tau) {(k \cdot MAD)}^2
\end{equation}

where $\tau$ still controls the weight between and $k$ sets to 1.4826, which is a widely used empirical value for estimating standard deviation. 


\begin{figure}[H]
\centering
\begin{tabular}{ccc}
  \includegraphics[width=0.32\textwidth]{Figures/IN_RBN/IN_RBN_Standard_R5.png} &
 \includegraphics[width=0.32\textwidth]{Figures/IN_RBN/IN_RBN_Salman_R5.png} &
  \includegraphics[width=0.32\textwidth]{Figures/IN_RBN/IN_RBN_Engstrom_R5.png}\\
  (a) Standard & (b) Salman et al.\cite{Salman2020DoAR} & (c) Engstrom et al. \cite{robustness}\\
\end{tabular}
	\caption{Corruption accuracy of leveraging median BN against our proposed attacks across $\tau$ and number of "$\tau$=1" layers. As a reference, Adapting test-time BN purely achieves 52.18\%, 53.50\%, and 53.14\% for Standard, Salman et al., and Engstrom et al., respectively. [TTA method: Norm] }
	\label{Fig:INC_RBN}
\end{figure}


\smallskip\noindent\textbf{Median BN demonstrates a comparable corruption accuracy with the common Norm method with a proper $\tau$ selection (Figure \ref{Fig:INC_RBN}).} We report the corruption accuracy of three models, where $\tau$ = \{0.1, 0.2, $\dots$, 1.0\} and the number of fully training-time BN layers is chosen from $N_{tr}$ = \{0, 1, 2, 4, 8, 16\}. It demonstrates that purely median BN ($\tau$=0.0) results in a significant performance drop in corruption accuracy (e.g., from 52.18\% to 13.15\% for the Standard model). However, adopting training-time BN and calibrating the median BN can boost the performance to a comparable accuracy with the Norm. As we can see, the best result for the Standard model can achieve 50.73\%. It is also worth noting that adversarially trained models (\cite{Salman2020DoAR,robustness}) exhibit similar behavior, especially for Engstrom et al., which even exceeds the Norm by 0.08\%. Therefore, we prove that by wisely combining training-time BN and median BN, models gain a similar benefit with the test-time BN method. 

\smallskip\noindent\textbf{Distribution Invading Attacks largely rely on the gradient information and cannot offer a reliable evaluation for median BN.} 
In our experiment, directly applying the distribution-invading attacks can hardly cause the median BN to misclassify the predictions. We hypothesize that the reason lies in the missing gradient of computing the median BN if controlled malicious samples do not contain middle values. 
\tw{maybe rephrase it to be more formal. (Also we need to show median is by nature more robust than mean)} 
As our main goal is to demonstrate the increasing vulnerabilities of TTA, we leave developing adaptive attacks of our median BN method for future studies. 


==> sections/discussion.tex <==
% \section{Discussion}

% As distribution shift frequently happens in real-world applications, leveraging test-time adaption is by far an effective and efficient mitigating approach. However, as our work showed, applying TTA exposes more vulnerabilities to malicious users than conventional ML systems. Therefore, we provide some suggestions for future deploying TTA from a security perspective:

% \begin{enumerate}
%     \item Only adopting batched test-time adaptation if all test data are from reliable sources. 
%     \item Leveraging single sample test-time adaptations \cite{Zhang2021MEMOTT,gao2022back} if not all collected test samples are reliable, distribution shifts.  
%     \item Constantly monitoring the model's performance and considering applying forensics on test inputs if necessary.  
% \end{enumerate}

% Aware of the attack

% Consider building a robust TTA method against potential malicious actors. 

